A Low-Cost Neural ODE with Depthwise Separable Convolution for Edge Domain Adaptation on FPGAs

High-performance deep neural network (DNN)-based systems are in high demand in edge environments. Due to its high computational complexity, it is challenging to deploy DNNs on edge devices with strict limitations on computational resources. In this paper, we derive a compact while highly-accurate DNN model, termed dsODENet, by combining recently-proposed parameter reduction techniques: Neural ODE (Ordinary Differential Equation) and DSC (Depthwise Separable Convolution). Neural ODE exploits a similarity between ResNet and ODE, and shares most of weight parameters among multiple layers, which greatly reduces the memory consumption. We apply dsODENet to a domain adaptation as a practical use case with image classification datasets. We also propose a resource-efficient FPGA-based design for dsODENet, where all the parameters and feature maps except for pre- and post-processing layers can be mapped onto on-chip memories. It is implemented on Xilinx ZCU104 board and evaluated in terms of domain adaptation accuracy, inference speed, FPGA resource utilization, and speedup rate compared to a software counterpart. The results demonstrate that dsODENet achieves comparable or slightly better domain adaptation accuracy compared to our baseline Neural ODE implementation, while the total parameter size without pre- and post-processing layers is reduced by 54.2% to 79.8%. Our FPGA implementation accelerates the inference speed by 23.8 times.

==> Makefile <==

# Makefile

# LATEX   = platex
LATEX   = pdflatex
BIBTEX  = pbibtex
DVIPS   = dvips
DVIPDF  = dvipdfmx
TARGET  = main
TEXFILE = $(TARGET).tex \
	refer.bib \
	settings.tex \
	abst.tex \
	intro.tex \
	related.tex \
	design.tex \
	impl.tex \
	eval.tex \
	conc.tex

all: $(TARGET).dvi

dvi: $(TARGET).dvi
$(TARGET).dvi: $(TEXFILE)
	$(LATEX) $(TARGET)
	$(BIBTEX) $(TARGET)
	$(LATEX) $(TARGET)
	$(LATEX) $(TARGET)

ps: $(TARGET).ps
$(TARGET).ps: $(TARGET).dvi
	$(DVIPS) -f $(TARGET).dvi > $(TARGET).ps

pdf: $(TARGET).pdf
$(TARGET).pdf: $(TARGET).dvi
	$(DVIPDF) $(TARGET).dvi

clean:
	rm -f $(TARGET).dvi
	rm -f $(TARGET).ps
	rm -f $(TARGET).log
	rm -f $(TARGET).pdf
	rm -f $(TARGET).bbl
	rm -f $(TARGET).blg
	rm -f *.aux *~ 



==> impl.tex <==

% impl.tex

\section{Implementation} \label{sec:impl}
% FPGA development at RTL level (Verilog / VHDL) usually requires a significant amount of human effort, limiting the applicability of FPGA-based accelerators.
% This is due to the intricacy of the algorithms, the necessity of manually tuning the synthesized design to fully exploit the FPGA's flexibility and implicit parallelism inherent in the algorithm, and the time-consuming verification process.
% High-level synthesis (HLS) is an automated process for synthesizing customized hardware from high-level languages including C/C++, which is advantageous and attractive in terms of improved productivity and rapid prototyping.
We implemented an IP core for the Greedy Endpoint Matching algorithm using Xilinx Vivado HLS v2019.1 toolchain.
We chose the Xilinx ZCU104 evaluation board as the target environment.
The clock frequency is set to 100 MHz.

Figure \ref{fig:scan-matching-ip-core} depicts an overview of our scan matching accelerator.
The module takes following as inputs from the software driver: (1) initial guess of pose $\{ x_t'^{[k]} \}$, (2) local map $\{ \widetilde{m}^{[k]} \}$ of all particles, (3) the latest sensor measurements $z_t = \{ z_t^i \}$, and (4) additional parameters, particularly the relative transformation of local map with respect to the entire map $\{ m^{[k]} \}$.
The top module consists of four submodules, each of which computes the refined pose $x_t^{[k]}$ for the $k$th particle based on scan matching, given the initial pose $x_t'^{[k]}$ and the local map $\widetilde{m}^{[k]}$.
As a result, scan matching processes for four different particles are executed simultaneously.
Throughout our implementation, all the decimal numbers are represented by 24-bit fixed-point format with 12-bit integer and 12-bit fractional parts or with 8-bit integer and 16-bit fractional parts.
Angular components $\{ \theta_t^i \}$ of the scan data $z_t$ can be computed from a minimum angle $\theta_0$ and an angular increment $\Delta \theta$ at the initialization phase, thus $\theta_t^i = \theta_0 + i \cdot \Delta \theta$.

It is worth mentioning that, in the software, the particle pose is optimized until reaching the convergence of the likelihood score, whereas in the hardware version, the number of iterations is fixed in exchange for the complete parallel execution.
Accordingly, the hardware scan matcher maintains constant latency cycles as long as the number of particles is fixed.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.9\linewidth]{fig/scan-matching-ip-core.pdf}
    \caption{Top Module for Scan Matching}
    \label{fig:scan-matching-ip-core}
\end{figure}


